Anchor Data Augmentation

We propose a novel algorithm for data augmentation in nonlinear over-parametrized regression. Our data augmentation algorithm borrows from the literature on causality and extends the recently proposed Anchor regression (AR) method for data augmentation, which is in contrast to the current state-of-the-art domain-agnostic solutions that rely on the Mixup literature. Our Anchor Data Augmentation (ADA) uses several replicas of the modified samples in AR to provide more training examples, leading to more robust regression predictions. We apply ADA to linear and nonlinear regression problems using neural networks. ADA is competitive with state-of-the-art C-Mixup solutions.

==> sections/CMixupExperiments.tex <==
In this section, we evaluate the performance of ADA and compare it to prior approaches on tasks involving both in-distribution and out-of-distribution generalization. We use the same datasets as \cite{yao2022cmix} and closely follow their experimental setup.\footnote{\cite{yao2022cmix} further assess task generalization. However the corresponding code was not publicly provided.} 

\textbf{Data: } We use four in-distribution datasets. For these data, the validation and test data are expected to follow the same distribution as the training data. Airfoil Self-Noise (Airfoil) and NO2 \citep{kooperberg1997statlib} are both tabular datasets, whereas Exchange-Rate and Electricity \citep{lai2018modeling} are timeseries datasets. We divide the datasets into train-, validation- and test data randomly. 

We use three datasets to evaluate out-of-distribution generalization, this means the validation and test data are no longer expected to be similarly distributed as the train set. First, we use RCFashion-MNIST (RCF-MNIST) \citep{yao2022cmix}, which is a synthetic modification of Fashion-MNIST that models subpopulation shifts. Second, we investigate domain shifts using Communities and Crime (Crime) and SkillCraft1 Master Table (SkillCraft) \citep{dua2019uci} both of which are tabular datasets. For Crime we use state identification and in SkillCraft we use "League Index", which correspond to different levels of competitors, as domain information. We split the datasets into train-, validation- and test data based on the domain information resulting in domain-distinct datasets. We provide a detailed description of datasets in Appendix \ref{app:cmixupexp}. 

\textbf{Models and comparisons: } We compare our approach, ADA, to C-Mixup \citep{yao2022cmix}, Manifold-Mixup \citep{verma2019manifold}, Mixup \citep{zhang2017mixup} and classical expected risk minimization (ERM). Following the work of \cite{yao2022cmix}, we use the same model architectures; That is a thee-layer fully connected network for the tabular datasets, LST-Attn \citep{lai2018modeling} for the timeseries and finally for ResNet-18 \citep{he2016deep} for RCF-MNIST. Since we follow the setup of \citep{yao2022cmix}, we apply CMixup, Manifold-Mixup, Mixup and ERM with their reported hyperparameters and provided code. In the ADA experiments we use hyperparametertuning and grid search to find the optimal training (batchsize, learning rate and number of epochs) and ADA parameters (number of clusters, range of $\gamma$ and whether to use manifold augmentation). We provide a detailed description in Appendix \ref{app:cmixupexp}. 

\textbf{@Shirin \& Fernando: this is a description of how I adapted ADA in the real datasets (I already mentioned all this in an earlier email). Feel free to move it into the appendix: \\
We cluster the entire training dataset into $k$ clusters. Then, we apply ADA on each batch using the corresponding cluster labels of the samples in the batch as an Anchor matrix and $\gamma$, which is randomly sampled from 20 values defined via the range of $\alpha$. Because the batches are likely to differ in each epoch due to random sampling, the model sees differently augmented samples in each epoch. }

On in-distribution datasets the evaluation metrics are Root Mean Squared Error (RMSE) and Mean Averaged Percentage Error (MAPE). Additionally, on out-of-distribution datasets we report the RMSE and the "worst" domain RMSE, which corresponds to the worst within-domain RMSE.

\textbf{Results: }

The results are presented in tables \ref{tab:realworlddata_indistr} and \ref{tab:realworlddata_ood}.


\begin{table}[ht!]
    \label{tab:realworlddata_indistr}
    \caption{Results for in-distribution generalization. We report the average RMSE and MAPE of three different seeds. Standard deviations are reported in \ref{app:cmixupexp}. Best results per column are printed bold and second best results are underlined.}
    \centering
    \begin{tabular}{lcccccccc}
    
    \toprule
         & \multicolumn{2}{c}{\textbf{Airfoil}} & \multicolumn{2}{c}{\textbf{NO2}} & \multicolumn{2}{c}{\textbf{Exchange- \newline Rate}} & \multicolumn{2}{c}{\textbf{Electricity}} \\
        \textbf{} & RMSE & MAPE & RMSE & MAPE & RMSE & MAPE & RMSE & MAPE \\ \midrule
        \textbf{ERM} & \underline{2.758} & 1.694 & 0.529 & 13.402 & \underline{0.024} & 2.437 & 0.058 & 13.915 \\ 
        \textbf{Mixup} & 3.264 & 1.964 & 0.522 & 13.226 & 0.025 & 2.513 & \underline{0.058} & 13.839 \\ 
        \textbf{ManiMixup} & 3.092 & 1.871 & 0.528 & 13.358 & 0.025 & 2.541 & 0.058 & 14.031 \\ 
        \textbf{CMixup} & 2.800 & \underline{1.629} & \underline{0.516} & \textbf{13.069} & 0.024 & \underline{2.431} & \textbf{0.057} & \underline{13.512} \\ \midrule
        \textbf{ADA} & \textbf{2.360} & \textbf{1.373} & \textbf{0.515} & \underline{13.128} & \textbf{0.021} & \textbf{2.116} & 0.059 & \textbf{13.464} \\
        \bottomrule
    \end{tabular}
\end{table}
\begin{table}[ht!]
    \label{tab:realworlddata_ood}
    \caption{Results for out-of-distribution generalisation. We report the average RMSE across domains in the test data and the "worst within-domain RMSE. Best results per column are printed bold and second best results are underlined.}
    \centering
   \begin{tabular}{lccccc}
    
    \toprule
        & \textbf{RCF-MNIST} & \multicolumn{2}{c}{\textbf{Crimes}} & \multicolumn{2}{c}{\textbf{SkillCraft}} \\ 
        \textbf{} & avg. RMSE & avg. RMSE & worst RMSE & avg. RMSE & worst RMSE \\ \midrule
        \textbf{ERM} & 0.164 & 0.136 & 0.170 & 6.147 & \underline{7.906} \\ 
        \textbf{Mixup} & 0.159 & 0.134 & 0.168 & 6.460 & 9.834 \\
        \textbf{ManiMixup} & \textbf{0.157} & \textbf{0.128} & \textbf{0.155} & \underline{5.908} & 9.264 \\
        \textbf{CMixup} & \underline{0.158} & 0.132 & 0.165 & 6.216 & 8.223 \\ \midrule
        \textbf{ADA} & 0.175 & \underline{0.130} & \underline{0.156} & \textbf{5.301} & \textbf{6.877} \\ \bottomrule
    \end{tabular}
\end{table}
    

==> sections/PoseEstimation.tex <==
In this section, we investigate the performance of ADA in deep learning using the example of pose estimation. We compare our approach to image augmentation techniques from computer vision. The goal of these experiments is not to improve or compare with existing benchmarks in pose estimation, but rather to investigate different augmentation techniques. Therefore, we apply ADA as it is without carefully  tuning the training hyperparameters.

\textbf{Data: }The following experiments are based on the MPII Human Pose dataset \cite{andriluka14humanpose}. It consists of images taken from a large variety of human activities with full-body pose annotations. In total $16$ bodily joints are annotated. We use the same training and validation datasets that are constructed in the work of \citet{sun2019deep} (also used in  \citet{xiao2018simple}). Hence, the training dataset is of size $n = 22 246$ and the validation one is of size $n = 2958$.

The images are sized to $(224 \times 224 \times 3)$ and normalized. In order to have a classical regression problem, the target is a $(16 \times 2)$- dimensional variable which corresponds to the $(x, y)$ coordinates of the respective joints in the image. This is in contrast to common pose estimation approaches, in which the output is a heatmap indicating the confidence of prediction of the location of each joint. 

\textbf{Models and Comparisons: } We use two different network architectures, both of which have pretrained vision networks followed by fully connected layers. In the first model, we use a pretrained Vision Transformer model with patch size $= 16$ which is trained on the ImageNet classification task \cite{imagenet15russakovsky} using the DINO method \cite{caron2021emergingproperties}. This is followed by three fully connected layers of sizes $(256, 64, 32)$. The second model uses a pretrained ResNet-50 architecture \cite{he2016deep}, which is also trained on ImageNet. This is followed by four fully connected layers of sizes $(512, 256, 128, 32)$. We freeze the vision networks (Dino and ResNet-50), so its main purpose is to extract (meaningful) features from the images and only the fully connected layers are optimized. This drastically decreases computational complexity. %We optimize using a mean squared error loss function and Adam optimization \cite{kingma2014adam}. We start with an initial learning rate of $0.001$, which is reduced every $5$ epochs by a multiplicative factor of $0.9$. We train for 150 epochs and use batchsize of $32$.

The two models are trained with different input data to investigate the effectiveness of ADA. We compare the following settings:

\begin{enumerate}
    \item \textit{No Augmentation}: The models are trained on original images only.
    \item \textit{Vanilla Augmentation}: The models are trained on original and vanilla augmented images including random scaling ($\pm 30 \%$), rotating ($\pm 30°$), and flipping. The annotations are also augmented accordingly.  
    \item \textit{ADA}: The models are trained on original images. After the vision models extract latent representations, we apply ADA for each minibatch. We sample $\gamma \sim U \left[0.5, 2\right]$ and use k-means clustering with $q = 2$ to construct $\mathbf{A}$.
    \item \textit{ADA + Global Clusters}: This approach is similar to ``ADA", except that one clustering ($q=2$) is computed on all samples instead of one clustering for each minibatch. The result of the global clustering is used to construct the anchor matrix for each minibatch.
    \item \textit{Vanilla Augmentation + Latent ADA}: This approach is similar to ``ADA", except that we start off using original and augmented images and subsequently perform our approach on the latent representations as described in the experiment ``ADA".
    \item \textit{Vanilla Augmentation + Image ADA}: The training data consists of original and augmented images. In addition to the vanilla augmentations, we further apply ADA on a minibatch of images using $\gamma \sim U\left[0.5, 2\right]$ and k-means clustering with $q = 2$ to construct $\mathbf{A}$. 
\end{enumerate}

\textbf{Results: } The results are presented in \Cref{tab:poseestimation_dino} and \Cref{tab:poseestimation_resnet}. We report the RMSE of the predictions on the resized images and the mean \textit{percentage of correct keypoints}, where the threshold for a joint prediction to be correct is $50\% \cdot $ of the headbone link (= PCKh@0.5). For RMSE lower and for PCKh@0.5 higher values correspond to better predictions. We observe that the Dino-based model achieves better predictions, suggesting that the obtained latent representations are more meaningful for the prediction task. Due to the simplifications in the model architecture and loss, our reported PCKh@0.5 are worse than the baseline pose estimations methods demonstrated e.g. \citet{xiao2018simple}. However, with ADA we are still able to see a marginal improvement in this measure in comparison to other baselines. %We believe futher improvements on a complicated task such as pose estimation can be achieved with ADA conditioned on more careful study  of the anchor matrix selection and analysis of it's effect on the implied robustness. We leave this to future work. %Yet, the mean PCKh@0.5 of all model settings is much worse than baseline pose estimation methods as demonstrated e.g. in. This suggests that the simplifications to the model architecture are not suitable and that the model is not capable of solving the pose estimation task effectively. This potentially also limits the improvements that can be achieved using augmentation techniques.

\begin{table}[H]
\caption{RMSE and mean PCKh@0.5 (in \%) for the Dino-based model architecture. Best-performing values are marked as bold.}
\label{tab:poseestimation_dino}
\centering
\begin{small}
\begin{sc}
\begin{tabular}{lcc}
\toprule
\makecell[l]{Experiment} & \makecell[c]{RMSE} & \makecell[c]{Mean \\ PCKh@0.5} \\
\midrule
\makecell[l]{No Augmentation }                             & 16.221 & 27.111 \\
\makecell[l]{Vanilla Augmentation}                         & 16.223 & 27.200 \\
\makecell[l]{ADA}     & 16.151 & 27.559 \\
\makecell[l]{ADA + Global Clustering}     & 16.167 & 27.520 \\
\makecell[l]{Vanilla Augmentation \\+ Latent ADA} & 15.975
& 28.556  \\
\makecell[l]{Vanilla Augmentation \\ + Image ADA}     &  \textbf{15.946}& \textbf{28.808} \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{table}

\begin{table}[H]
\caption{RMSE and mean PCKh@0.5 (in \%) for the ResNet-based model architecture. Best-performing values are marked as bold.}
\label{tab:poseestimation_resnet}
\centering
\begin{small}
\begin{sc}
\begin{tabular}{lcc}
\toprule
\makecell[l]{Experiment} & \makecell[c]{RMSE} & \makecell[c]{Mean \\ PCKh@0.5} \\
\midrule
\makecell[l]{No Augmentation }                             & 16.719 & \textbf{27.195} \\
\makecell[l]{Vanilla Augmentation}                         & 16.645 & 26.406 \\
\makecell[l]{ADA}     & \textbf{16.520} & 26.987 \\
\makecell[l]{ADA + Global Clustering}     & 16.545 & 27.062 \\
\makecell[l]{Vanilla Augmentation  \\+ Latent ADA} & 16.686 & 26.620  \\
\makecell[l]{Vanilla Augmentation \\ + Image ADA} & 16.756 & 26.084  \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{table}


==> sections/RelatedWork_OLD.tex <==
Many different data augmentation methods have been proposed in recent years with varying applications in mind. Still most augmentations we mention here use human-designed transformations with domain knowledge, which leaves the target variable invariant. For instance, Cutout \citep{devries2017improved} is an image-specific augmentation technique that is successfully used to train models on CIFAR10 and CIFAR100 \cite{krizhevsky2009learning} but was determined to be unsuitable for larger image datasets like ImageNet with higher resolution \cite{deng2009imagenet}. Other augmentation methods for images such as random crop, horizontal or vertical mirroring, random rotation or translation \cite{lecun1998gradient,simonyan2014very} may similarly apply to a certain group of image datasets while being inapplicable to others, e.g. datasets of digits and letters. 

In an attempt to automate the augmentation process and reduce human involvement, policy or search-based automated augmentation methods were developed. In AutoAugment \cite{cubuk2019autoaugment} a neural network is trained with Reinforcement Learning (RL) to combine an assortment of transformations in varying strengths to apply on samples of a given dataset and improve the model accuracy. The following work aims at reducing the cost of the pretraining search phase in automated augmentation with randomized transformations and reduced search space (RandAugment \cite{cubuk2020randaugment}, Fast AutoAugment \cite{lim2019fast}, UniformAugment \cite{lingchen2020uniformaugment} and TrivialAugment \cite{muller2021trivialaugment}), continuous action space and differentiable transformations (Faster AutoAugment \cite{hataya2020faster} and DADA \cite{li2020differentiable}).

Alternatively, to adapt the augmentation policy to the model during training, Population-Based Augmentation \cite{ho2019population} and Online Hyperparameter Learning \cite{lin2019online} use multiple data augmentation workers who are updated using evolutionary strategies and RL, respectively. 
Adversarial AutoAugment \cite{zhang2019adversarial} and AugMax \cite{wang2021augmax} optimize for the augmentation policy that deteriorates the training accuracy and improves its robustness. and Augmentationwise Weight Sharing \cite{tian2020improving} based on RL in the last stages of training. DivAug \cite{liu2021divaug} finds the policy which maximized the diversity of the augmented data.

Having a separate search phase for optimal augmentation policy is computationally expensive and may exceed the required computation to train the downstream model \cite{xu2022universal, cubuk2020randaugment}. In addition, these methods and their online counterparts need to be trained separately on every single dataset. While OnlineAugment \cite{tang2020onlineaugment} and DDAS exploit meta-learning to avoid this problem, they still rely on a set of predefined class invariant transformations that require domain-specific information.

Generic transformations such as Gaussian or adversarial noise \cite{devries2017improved, taylor2018improving, lakshminarayanan2017simple} and dropout \cite{bouthillier2015dropout} is also effective in expanding the training dataset. Generative models such as Generative Adversarial Networks (GAN) \cite{goodfellow2020generative} and Variational Auto-Encoders (VAE) \cite{kingma2013auto} are trained in \cite{antoniou2017data,chadebec2021data, tang2020onlineaugment} to synthesize samples close to the low dimensional manifold of the data for classification. 

More recently, Mixup \cite{zhang2017mixup} proposed a popular data augmentation by using a convex combination of pairs of samples from different classes and their softened labels for augmentation. The procedure is only illustrated for classification problems, even when it is mentioned in the discussion that the application to regression is straightforward. Various extensions of Mixup have been proposed to prevent data manifold intrusion \cite{verma2019manifold}, use more complex mixing \cite{yun2019cutmix} account for saliency in augmented samples \cite{kim2021co, kim2020puzzle}. These methods were predominantly designed to excel in classification tasks. In particular, Mixup for regression was studied in \cite{carratino2020mixup, zhang2020does, hwang2021regmix} but it was observed to adversely impact the predictions in regression problems when misleading augmented samples are generated from pair of faraway samples. In \cite{carratino2020mixup} and \cite{zhang2020does}, Mixup is studied theoretically as a regularization technique applicable to both regression and classification problems, but the algorithm is only illustrated for classification problems. \cite{hwang2021regmix} is the only paper that studies data augmentation for regression and, it was detailed in our paper’s introduction.

%More recently, Mixup \cite{zhang2017mixup} proposed a popular data augmentation by using a convex combination of pairs of samples from different classes and their softened labels for augmentation. Various extensions of Mixup have been proposed to prevent data manifold intrusion \cite{verma2019manifold}, use more complex mixing \cite{yun2019cutmix} account for saliency in augmented samples \cite{kim2021co, kim2020puzzle}. These methods were predominantly designed to excel in classification tasks. In particular, Mixup for regression was studied in \cite{carratino2020mixup, zhang2020does, hwang2021regmix} but was observed to adversely impact the predictions in regression problems when misleading augmented samples are generated from pair of far away samples. This was overcome in RegMix \cite{hwang2021regmix} using neighborhood information to mix the samples.

%As opposed to Mixup and most of its variants, our method combines multiple data samples to generate a single augmented data. 



